Simultaneous Frequentist Calibration of Confidence Regions for Multiple Functionals in Constrained Inverse Problems

Many scientific analyses require simultaneous comparison of multiple functionals of an unknown signal at once, calling for multidimensional confidence regions with guaranteed simultaneous frequentist under structural constraints (e.g., non-negativity, shape, or physics-based). This paper unifies and extends many previous optimization-based approaches to constrained confidence region construction in linear inverse problems through the lens of statistical test inversion. We begin by reviewing the historical development of optimization-based confidence intervals for the single-functional setting, from "strict bounds" to the Burrus conjecture and its recent refutation via the aforementioned test inversion framework. We then extend this framework to the multiple-functional setting. This framework can be used to: (i) improve the calibration constants of previous methods, yielding smaller confidence regions that still preserve frequentist coverage, (ii) obtain tractable multidimensional confidence regions that need not be hyper-rectangles to better capture functional dependence structure, and (iii) generalize beyond Gaussian error distributions to generic log-concave error distributions. We provide theory establishing nominal simultaneous coverage of our methods and show quantitative volume improvements relative to prior approaches using numerical experiments.

==> miscellaneous/temporary-251012.tex <==
\section{Conclusion and open directions}

\paragraph{Summary of contributions.}
We introduced a unified test–inversion framework for confidence regions in linear inverse problems with linear or conic constraints.
Our analysis ties three statistics---$\lambda^2_c$, $\lambda^2_u$, and $\lambda^1$---to concrete optimization templates and calibration rules.
We established convexity and recession–monotonicity for $\lambda^2_u$ and $\lambda^1$, identified where their worst–case quantiles occur, and gave tight stochastic dominance relations.
We proved that, over closed convex cones, the maximizing quantiles for $\lambda^2_u$ and $\lambda^1$ occur at $x=0$ and admit $\bar\chi^2$ laws, with linked intrinsic–volume weights.
We developed practical high–dimensional methods: refined TFM reductions, multi–functional generalizations, box–constraint reductions, and a row/null splitting strategy.
We supplied optimal global thresholds for nonnegative problems for $\lambda^2_u$ and $\lambda^1$, improving classical $\chi^2$ bounds and Burrus–style intervals.

\paragraph{Practical guidance.}
Prefer the $\mu$–description over the $x$–box whenever feasible, as it yields strictly smaller regions at the same coverage.
For nonnegative problems, calibrate $\lambda^2_u$ or $\lambda^1$ at the origin and use the resulting optimal global constant.
Expect $\lambda^2_u$ to give shorter average radii for small $\alpha$ but a worse worst–case than $\lambda^1$.
Use the row/null split when $H$ has components outside $\row(K)$: treat the row part with a Gaussian ellipsoid (or its constrained counterpart) and the null part with strict–bounds–type sets, combining them via a Minkowski sum.
Apply the generalized TFM reductions when $k\ll p$ and the sign–splits of $H$ lie in $\row(K)$ (or can be implemented via pseudoinverses).

\paragraph{Beyond Gaussian noise.}
All convex–analytic results (quantile convexity for $\lambda^1$, recession–monotonicity, extremal structure, and boundedness tests) extend to log–concave noise by replacing least–squares loss with $-2\log p(y\mid x)$ \cite{BatlleDisproof}.
Under log–concavity, $\lambda^1$ remains tractable and convex by Prékopa’s theorem, whereas $\lambda^2_u$ generally loses convexity when the least–squares Pythagorean identity disappears.
Exact $\chi^2$ and $\bar\chi^2$ laws are no longer available, but origin–quantiles are still estimable via convex programs and Monte Carlo.

\paragraph{Chance–constrained calibration avenues.}
Direct calibration of the likelihood–ratio statistic $\lambda^2_c$ can be posed as a chance–constrained program (CCP) \cite{BatlleDisproof}.
Scenario methods \cite{Nemirovski2006,campi_garatti_2011} provide nonasymptotic feasibility guarantees at the cost of additional constraints and potential conservatism.
Convex surrogates replace Value–at–Risk by CVaR \cite{cvar_paper}, or use broader convex approximations for CCPs \cite{convex_approx_ccp}, yielding tractable programs with explicit certificates.
These tools are attractive when analytic quantiles are unavailable, but they need careful validity checks in finite samples.

\paragraph{Design of alternative statistics.}
It may be fruitful to design test statistics whose induced CCPs are convex by construction.
For log–concave noise, quasi–concave test statistics in the parameter can yield convex feasibility regions by results in \cite{prekopa2003}.
While $\lambda^1$ already fits this template, we expect other choices to trade statistical power, robustness, and computational ease in useful ways.

\paragraph{Special cases and revived conjectures.}
Although the Burrus conjecture fails in general, empirical successes suggest structured regimes where $\chi^2_1$ thresholds might still be valid \cite{patil2022,stanley_unfolding,stanley2025confidenceintervalsfunctionalsconstrained}.
Promising cases include specific $(K,h)$ geometries, asymptotic regimes with large $n$ and/or $p$, and interior points well separated from the constraint boundary.
Characterizing such regimes would sharpen practice while respecting known counterexamples.

\paragraph{Broader impact on constrained inference.}
Our approach may reduce conservatism in strict–bounds style confidence bands used in shape–restricted problems \cite{stark_strict_bounds,hengartner_stark_1995}.
The chi–bar–squared perspective and intrinsic–volume links extend beyond classical Type A/B settings \cite{Silvapulle2001}, potentially informing modern constrained M–estimation and projection–based procedures.

\paragraph{Open problems.}
Derive structural or partial maximization results for the $\lambda^2_c$ quantile under linear or conic constraints.
Compare $\lambda^2_u$ versus $\lambda^1$ systematically via their $\bar\chi^2$ origin laws to obtain decision rules based on $(K,H)$ geometry.
Tighten finite–sample uniform bounds beyond $\chi^2_{\rank(K)}$ when additional structure is available.
Develop fast, reliable origin–quantile estimators in high dimensions with rigorous error control.
Optimize the Bonferroni split in row/null decomposition beyond the equal–split default.
Extend reductions and split methods to mixed noise models (e.g., sub–Gaussian tails or heteroskedasticity) while preserving tractability and coverage.
Characterize classes of $(K,H,\mathcal X)$ where sliced optima $d^*(\mu)$ admit closed forms or certified approximation schemes.

\paragraph{Closing remark.}
The unifying view offered here clarifies when and how to obtain valid, sharp, and computationally tractable confidence regions, and it opens several concrete paths to push constrained inference beyond the Gaussian least–squares frontier.

